The Waymo Open Sim Agents Challenge

Simulation with realistic, interactive agents represents a key task for autonomous vehicle software development. In this work, we introduce the Waymo Open Sim Agents Challenge (WOSAC). WOSAC is the first public challenge to tackle this task and propose corresponding metrics. The goal of the challenge is to stimulate the design of realistic simulators that can be used to evaluate and train a behavior model for autonomous driving. We outline our evaluation methodology, present results for a number of different baseline simulation agent methods, and analyze several submissions to the 2023 competition which ran from March 16, 2023 to May 23, 2023. The WOSAC evaluation server remains open for submissions and we discuss open problems for the task.

==> tex/component_metrics_val.tex <==
\begin{table*}[!h]
    \caption{Per-component metric results on the \emph{validation} split of WOMD, representing likelihoods. Methods are ranked by composite metric; Numbers within 1\% of the best are in bold (excluding `logged oracle'). Note: * indicates an invalid submission, not executed fully in closed-loop.}
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begingroup
    %\renewcommand{\arraystretch}{1.25}
    \begin{tabular}{l|cccccccccc|cc}
    \toprule
\rowcolorize \textsc{Agent Policy}	& \textsc{linear}	& \textsc{linear }	& \textsc{ang.}	& \textsc{ang.}	& \textsc{dist.}	& \textsc{collision}	& \textsc{TTC} &	\textsc{dist. to} &	\textsc{offroad} & \textbf{\textsc{Composite}}	& \textsc{ADE}	& \textsc{minADE}	 \\
\rowcolorize \textsc{}	& \textsc{speed}	& \textsc{accel.}	& \textsc{speed}	& \textsc{accel.}	& \textsc{to obj.}	& \textsc{}	& \textsc{} &	\textsc{road edge} &	\textsc{} & \textbf{\textsc{Metric}($\uparrow$)}	& \textsc{($\downarrow$)}	& \textsc{($\downarrow$)}	 \\

\midrule
\textsc{Random Agent}                                       & 0.002 & 0.046 & 0.073 & 0.120 & 0.003 & 0.005 & 0.735 & 0.187 & 0.333 & 0.166 & 50.935 &	50.796 \\
\rowcolorize \textsc{Constant Velocity}                     & 0.075 & 0.058 & 0.019 & 0.034 & 0.207 & 0.207 & 0.739 & 0.453 & 0.319 & 0.237 & 7.916 & 7.916 \\
 \textsc{Constant Velocity (+ Gaussian Noise)}  & 0.159	& \textbf{0.119}	& 0.019	& 0.034	& 0.199	& 0.258	& 0.778	& 0.473	& 0.356	& 0.271 & 7.575	& 7.221	 \\
\rowcolorize \textsc{Wayformer* (Identical Samples)}	                    & 0.336	& 0.098	& 0.412	& 0.406	& 0.227	& 0.342	& 0.772	& 0.483	& 0.473	& 0.393 & \textbf{2.493}	& 2.493	 \\
 \textsc{Wayformer* (Diverse Samples)} 	        & \textbf{0.410}	& \textbf{0.127}	& \textbf{0.473}	& \textbf{0.437}	& \textbf{0.354}	& \textbf{0.385}	& \textbf{0.796}	& \textbf{0.527}	& \textbf{0.507} 	& \textbf{0.442} & 2.592	& \textbf{1.704}	 \\
\bluerowcolorize\textsc{Logged Oracle}	                & 0.562	& 0.330	& 0.565	& 0.489	& 0.973	& 1.000	& 0.883	& 0.707	& 1.000	& 0.766 & 0.000	& 0.000  \\
    \bottomrule
    \end{tabular}
    \endgroup
    \end{adjustbox}
    \label{tab:per-metric-scores-val}
\end{table*}


==> tex/neurips_checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} % See Section \ref{sec:societal-impacts}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{} % Available at https://nips.cc/public/EthicsGuidelines
\end{enumerate}




\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{For the most part, yes. Both our evaluation code and WOMD \cite{Ettinger21iccv_WOMD} are publicly available. In addition, several external submissions to the Challenge have open-source code, and submission files could be reproduced via model inference. However, we have not publicly released the uploaded submission files. Wayformer \cite{Nayakanti23icra_Wayformer} is a proprietary model and is not publicly available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{No new models were trained for this benchmark.} %\textcolor{red}{Ask Ben, Drago, Rami regarding this, or just cite the Wayformer paper.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{No, as the evaluation is deterministic and does not utilize a seed. However, users submitted many diverse rollouts for each simulated scene using various seeds, and all such rollouts are used in our evaluation.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See Section A.3 of the Supplementary Material.}
    % WOMD license -> 
    % WOSAC eval code -> https://github.com/waymo-research/waymo-open-dataset/blob/master/src/waymo_open_dataset/wdl_limited/sim_agents_metrics/LICENSE
    
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See Section A.3 of the Supplementary Material for a description of the evaluation code, as well as links to its source files on Github.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

